S-CLIP: Semi-supervised Vision-Language Learning using Few Specialist Captions

Vision-language models, such as contrastive language-image pre-training (CLIP), have demonstrated impressive results in natural image domains. However, these models often struggle when applied to specialized domains like remote sensing, and adapting to such domains is challenging due to the limited number of image-text pairs available for training. To address this, we propose S-CLIP, a semi-supervised learning method for training CLIP that utilizes additional unpaired images. S-CLIP employs two pseudo-labeling strategies specifically designed for contrastive learning and the language modality. The caption-level pseudo-label is given by a combination of captions of paired images, obtained by solving an optimal transport problem between unpaired and paired images. The keyword-level pseudo-label is given by a keyword in the caption of the nearest paired image, trained through partial label learning that assumes a candidate set of labels for supervision instead of the exact one. By combining these objectives, S-CLIP significantly enhances the training of CLIP using only a few image-text pairs, as demonstrated in various specialist domains, including remote sensing, fashion, scientific figures, and comics. For instance, S-CLIP improves CLIP by 10% for zero-shot classification and 4% for image-text retrieval on the remote sensing benchmark, matching the performance of supervised CLIP while using three times fewer image-text pairs.

==> backup.tex <==
% Vision-language pre-training~\citep{bommasani2021opportunities} has demonstrated remarkable success, achieving new state-of-the-art results in many vision and language problems. One representative method is contrastive language-image pre-training (CLIP)~\citep{radford2021learning}, which uses contrastive learning to learn a joint embedding of text and images. The training objective of CLIP involves solving two classification tasks: predicting the text that corresponds to an image, and vice versa, finding the matching instance from a batch of image-text pairs. As a result, CLIP learns to interchange the image and text embeddings, enabling various downstream tasks such as zero-shot classification and image-text retrieval.

% Despite their success, CLIP and other vision-language models face challenges in specialized domains such as remote sensing or medical imaging~\citep{kim2023explaining}. The primary issue is the lack of sufficient annotated image-text pairs, which limits the pre-training of models in these domains. To address this challenge, previous research has mainly focused on constructing large-scale datasets of image-text pairs for each domain~\citep{johnson2019mimic, yang2020fashion}. However, annotating data for each specialized domain can be time-consuming and expensive, limiting its applicability to various domains. For example, to the best of our knowledge, public datasets for remote sensing images have only 15,000 available pairs~\citep{arampacha2021fine}.

% In other fields of machine learning, particularly for image classification, semi-supervised learning~\citep{chapelle2006semi} is a popular approach for learning a model using limited annotations. Semi-supervised learning typically relies on pseudo-labeling~\citep{lee2013pseudo}, which predicts pseudo-labels for unlabeled data by propagating information from labeled data and refines the model using predicted pseudo-labels. This approach, combined with self-supervised learning, which learns representations from unlabeled data, has significantly improved classifiers using only a few class labels~\citep{berthelot2019mixmatch, sohn2020fixmatch, assran2021semi, bovsnjak2023semppl}.




% \begin{table*}[t]
% \centering\fontsize{8.5pt}{8.5pt}\selectfont
% % \centering\small
% \caption{%
% Zero-shot classification results on fashion datasets. Parentheses indicate the performance gap from the supervised baseline,
% % where values highlighted in green indicate gaps larger than 0.5.
% % We compare the original CLIP, supervised CLIP fine-tuned on labeled data (L), and semi-supervised methods.
% }\label{tab:fashion-zeroshot}
% \vspace{-0.08in}
% % \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{lcccc}
% \toprule
% % \vspace{0.03in}
% Method & FashionGen & FACAD & Fashion200k & PolyvoreOutfits \\
% \midrule
% CLIP (original) & 
% xx.x\blankstdv\blankup & xx.x\blankstdv\blankup & xx.x\blankstdv\blankup & xx.x\blankstdv\blankup \\
% \midrule
% CLIP (fine-tune) &
% \\
% \midrule
% Hard-PL &
% \\
% Soft-PL &
% \\
% S-CLIP (ours) &
% \\
% %
% \bottomrule
% \end{tabular}
% % \end{adjustbox}
% \end{table*}


% \begin{table*}[t]
% \centering\small
% \caption{%
% Zero-shot classification and image-text retrieval results on Fashion200k dataset. Bolds denote the best results.
% \tbd{tbd}
% }\label{tab:fashion}
% \vspace{-0.08in}
% % \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{lcccccc}
% \toprule
% & \multicolumn{2}{c}{Zero-shot} & \multicolumn{2}{c}{Image$\to$text} & \multicolumn{2}{c}{Text$\to$image} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
% % \vspace{0.03in}
% Method & SUB-CLS & CLS & R@5 & R@10 & R@5 & R@10 \\
% \midrule
% CLIP (original) & 
% 29.3\blankstdv & 73.4\blankstdv &
% 10.8\blankstdv & 16.0\blankstdv &
% 10.1\blankstdv & 15.1\blankstdv \\
% \midrule
% CLIP (fine-tune) &
% 37.4\stdv{0.7} & 78.4\stdv{0.9} &
% 13.7\stdv{0.3} & 20.5\stdv{0.3} &
% 14.0\stdv{0.2} & 20.7\stdv{0.1} \\
% \midrule
% %
% Hard-PL \\
% Soft-PL \\
% S-CLIP (ours) &
% \textbf{38.9}\stdv{0.5} & \textbf{80.7}\stdv{0.6} & 
% \textbf{13.9}\stdv{0.6} & \textbf{20.8}\stdv{1.0} & 
% \textbf{14.1}\stdv{0.4} & \textbf{21.1}\stdv{0.6}  \\
% %
% \bottomrule
% \end{tabular}
% % \end{adjustbox}
% \end{table*}


% \begin{table*}[t]
% \centering\fontsize{8.5pt}{8.5pt}\selectfont
% % \centering\small
% \caption{%
% Zero-shot classification and image-text retrieval results on Fashion200k dataset. Bolds denote the best results.
% \tbd{tbd}
% }\label{tab:fashion}
% \vspace{-0.08in}
% % \begin{adjustbox}{width=\linewidth}
% \begin{tabular}{lcccccc}
% \toprule
% % \vspace{0.03in}
% Method & Fashion200k & Fashion200k (SUB) & FashionGen & PolyvoreOutfits \\
% \midrule
% CLIP (original) & 
% 73.4\blankstdv & 29.3\blankstdv & 35.9\blankstdv & 58.4\blankstdv \\
% \midrule
% CLIP (fine-tune) &
% 80.3\stdv{1.1} & 39.4\stdv{0.4} & 49.4\stdv{2.9} & 67.8\stdv{3.3} \\
% \midrule
% Hard-PL &
% 79.2\stdv{0.6} & 38.2\stdv{0.9} & 49.0\stdv{1.4} & 69.3\stdv{1.4} \\
% Soft-PL &
% 79.8\stdv{1.7} & 38.4\stdv{0.6} & 48.1\stdv{2.1} & 75.3\stdv{2.6} \\
% S-CLIP (ours) &
% \textbf{82.1}\stdv{0.7} & \textbf{39.5}\stdv{1.0} & 
% \textbf{56.6}\stdv{1.8} & \textbf{73.7}\stdv{2.8} \\
% %
% \bottomrule
% \end{tabular}
% % \end{adjustbox}
% \end{table*}
